SciWING -- A Software Toolkit for Scientific Document Processing

We introduce SciWING, an open-source software toolkit which provides access to pre-trained models for scientific document processing tasks, inclusive of citation string parsing and logical structure recovery. SciWING enables researchers to rapidly experiment with different models by swapping and stacking different modules. It also enables them declare and run models from a configuration file. It enables researchers to perform production-ready transfer learning from general, pre-trained transformers (i.e., BERT, SciBERT etc), and aids development of end-user applications. It includes ready-to-use web and terminal-based applications and demonstrations (Available from http://sciwing.io).

==> SciWING - SDP/comments/comments.emnlpdemo.tex <==
Dear Abhinav Ramesh Kashyap:

I am sorry to inform you that the following submission was not selected by the program committee to appear at EMNLP - Demonstrations 2020:

SciWING - A Software Toolkit for Scientific Document Processing

The selection process was very competitive. Due to time and space limitations, we could only choose a small number of the submitted papers to appear on the program. Nonetheless, I still hope you can attend the conference.

I have enclosed the reviewer comments for your perusal.

If you have any additional questions, please feel free to get in touch.

Best Regards,
David Schlangen and Qun Liu
EMNLP - Demonstrations 2020

============================================================================ 
EMNLP - Demonstrations 2020 Reviews for Submission #83
============================================================================ 

Title: SciWING - A Software Toolkit for Scientific Document Processing
Authors: Abhinav Ramesh Kashyap and Min-Yen Kan


============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 4
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 5
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper describes a toolkit for scientific document processing. It allows several NLP tasks such as reference string parsing, scienceIE, and I2B2 NER. It provides CLI, Python, and Web API.

STRENGTHS:
1. The software is easy to use (can be installed using pip) with lots of examples. It provides many interfaces and can be customized/extended easily.
2. The demo site (which is different from the one written in this paper) vividly shows how this toolkit can be used to perform scientific document processing.
3. It contains up-to-date pre-trained models and is actively maintained.

WEAKNESSES:
1. The development of the software is mainly done by a single person (the first author of this paper). It would be great if the software can be maintained by a group of people (it is often the case that software will become unmaintained after the initial release if the person lost his interest/becomes busy/etc.). 
2. (probably related to the previous point) It is hard to keep the environment up-to-date. It is better to "freeze" the versions of deep learning toolkits and libraries because otherwise "pip install" often breaks (From my experience, I have to update the versions of CUDA and PyTorch every year unless I pin down the versions, otherwise the software won't work as expected). 
https://github.com/abhinavkashyap/sciwing/issues/22

Style:
The code snippet in this paper looks a bit strange. I would suggest using a different font.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 3
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 1
                    Recommendation (1-5): 3
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper presents SciWING, a platform that supports SDP tasks. One of the main goals is to provide a flexible framework to support SDP tasks for non-NLP experts by providing pre-trained models for scientific data. The authors compare with existing frameworks and present a clear motivation for the work. They show how to configure the system, and discuss several related tasks.

Strength:

- The authors did extensive work on the SciWING APIs
- The technical description of the system and how to use it is well detailed and explained

Weaknesses:

- The authors claim that the platform is for non-NLP experts that wish to do some research on Scientific data. Given this, does your system provide suggestions or recommendations of what components are "making sense" to use during the building part?
- Some details and choices are not entirely clear:
o For the Logical Structure recovery task - how it was trained, which data was used?
o although the authors mention in the future work the task of Summarization (as part of generation), it seems to be one of the important and recent tasks comparing for example with niche tasks such as citation intent classification. Thus it is not clear what was the criteria for the chosen tasks.
- In order to fully understand the platform capabilities, it would be nice to show how general is the system by, for example, showing for NER is also perform on different datasets such as BC5CDR or NCBI-disease.
- Although a demo link was provided it was not accessible (during several different times that I've checked)
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 2
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 3
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 3
                    Recommendation (1-5): 2
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper presents a tool for scientific document processing.  While this is an important and somewhat understudied problem domain, I feel like the paper makes claims that are unsubstantiated or inadequately defined, and it also does not sufficiently clarify its unique contributions over existing work. While the idea of a user-friendly and state-of-the-art scientific document processing library is perhaps a worthy goal, SciWING may need further refinement before it is ready to be presented as a demo at EMNLP.

Table 1 is very important -- it makes strong claims about the advantages of SciWING over existing toolkits.  Thus, it’s problematic that the columns of that table (corresponding to qualities that the paper claims SciWING has and previous toolkits lack) are not defined in the paper.  What does “neural-first” mean, in terms of what one can do with the toolkit?  What qualifies as “extensible”?  What workload do the authors use to claim that their approach is “SOTA” and none of the others are?

I was also not clear on what SciWING offers that differs from the base capabilities in AllenNLP.  Most of what the paper mentions in Section 2 -- the models, the training and testing capability, tokenizers, logging, metrics, support for embeddings, seem like AllenNLP components.  The TOML configuration file seems like an analogue to AllenNLP configuration files, albeit in a slightly different format.  Taking capabilities from AllenNLP makes perfect sense -- but the paper needs to be much more clear on what capabilities are new in this tool, versus built-in to AllenNLP.

Finally, related to my question about Table 1, I also found it confusing that the paper refers to itself as “SOTA” and all other tools as “not SOTA”, given that SciWING underperforms the state of the art in three of the four tasks where a comparison is made in Table 2.  Some of these performance gaps seem practically significant (e.g., the 2% absolute increase in reference parsing error seems like it would drive practitioners to use another tool instead -- can the authors bring this number up by incorporating other approaches?).
---------------------------------------------------------------------------




==> SciWING - SDP/comments/comments.sdp.tex <==
============================================================================ 
SDP 2020 Reviews for Submission #17
============================================================================ 

Title: SciWING– A Software Toolkit for Scientific Document Processing
Authors: Min-Yen Kan and Abhinav Ramesh Kashyap


============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 2
           Soundness / Correctness (1-5): 4
             Meaningful Comparison (1-5): 2
                      Thoroughness (1-5): 2
        Impact of Ideas or Results (1-5): 3
                    Recommendation (1-5): 3
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
The paper presents SYS, an open source toolkit that packages existing models for scientific document processing.  The toolkit provides access to both a command-line interface and a web interface.

The tool aims to provide immediate access to SOTA models for scientific NLP.  My main concern with the paper is that the main claimed benefit with respect to other toolkits is that it provides access to SOTA models (with respect to those provided by other toolkits like AllenNLP, SciSpaCy, etc.)  But the paper doesn't include any empirical results to support this claim.  Also, I assume these are all moving targets as different toolkits incorporate new and better models.

In any event, I do think there is some value in having more innovation in toolkits that provide easy access to NLP models, so there is some merit to this work.  This is a more like a demo paper than a traditional workshop paper presenting new empirical results, but I do think it fits the theme of the workshop.

One other concern: the paper does include links to the toolkit and demo that break anonymity.  In general, I think it is better to use an anonymized URL, or provide sample outputs as supplementary materials for double-blind reviewing.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 3
           Soundness / Correctness (1-5): 3
             Meaningful Comparison (1-5): 4
                      Thoroughness (1-5): 4
        Impact of Ideas or Results (1-5): 4
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
The authors propose a software toolkit for several SDP tasks. It is made
freely available online. As a modular architecture is chosen and
existing, well established components are being used, the general
approach taken seems sound. Referring to recent related work, the
authors properly position their work within the context of existing
literature. The key points of motivation for developing a new software
are (1) existing software being either too general (no SDP focus) or too
specific (e.g. for a certain scientific domain), and (2) the fact that
existing software is argued to be insufficiently accessible.
Pre-trained models integrated in the toolkit are evaluated against
existing approaches, where the proposed software is observed to achieve
a performance close to the state of the art. Given that SOTA components
appear to be integrated as is, this isn't much of a surprise.

In terms of presentation the proposed toolkit is described clearly and
the document structure is sound. Parts of section 2, however, read a bit
like a software documentation. Maybe the section could have been more
concise and the freed up space then used to discuss other aspects like
the toolkit's extensibility (e.g. ease of adding in a new data set or
embedding model).

While part of the motivation is the domain specificity of existing
software, some components of the proposed toolkit (for ScienceIE, I2B2,
and NER) appear to be domain specific as well.

Lastly, section 4 ends somewhat abruptly. A little discussion concerning
the listed use cases would have been helpful.

Overall, the presented work seems solid, but it is somewhat hard to give
a clear verdict, as no useful quantitative comparison to existing
software seems possible. The paper might be worth accepting, because the
tool appears useful and it would be interesting to see the community's
take on it.

Minor points:
- In Table 2 the toolkit is called "SciWING" instead of "SYS"
- Typo at the end of section 5: "provide access" -> "provides access"
---------------------------------------------------------------------------


Questions for Authors
---------------------------------------------------------------------------
1. Concerning datasets you argue that your toolkit unifies various input
formats. Can you elaborate on what this means for integrating further
data sets into the toolkit?
2. What was the reason for choosing the TOML format for configuration files?
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 4
           Soundness / Correctness (1-5): 5
             Meaningful Comparison (1-5): 5
                      Thoroughness (1-5): 4
        Impact of Ideas or Results (1-5): 4
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
I would have appreciated a more in-depth analysis of the scalability/efficiency of SYS (currently and in the future), when facing processing of very large amounts of documents.
---------------------------------------------------------------------------

==> SciWING - SDP/comments/comments.tex <==
Reviewer question ends in ---------
Our response ends in ========

---START---

Lastly, section 4 ends somewhat abruptly. A little discussion concerning
the listed use cases would have been helpful.
-----------------------------------------------------------------------------------------
 Abhi - Added one paragraph at the end of section 4 to conclude 
=====================================================================================


I was also not clear on what SciWING offers that differs from the base capabilities in AllenNLP.  Most of what the paper mentions in Section 2 -- the models, the training and testing capability, tokenizers, logging, metrics, support for embeddings, seem like AllenNLP components.  The TOML configuration file seems like an analogue to AllenNLP configuration files, albeit in a slightly different format.  Taking capabilities from AllenNLP makes perfect sense -- but the paper needs to be much more clear on what capabilities are new in this tool, versus built-in to AllenNLP.
---------------------------------------------------------------------------------------
Abhi - Addressed this by saying that we want to encourage researchers to minimally change an architecture and experiment vs AllenNLP which expects researcher to understand complex abstractions
=========================================================================================



What was the reason for choosing the TOML format for configuration files?
-------------------------------------------------------------------------------------
Abhi - It is widely used and is easy to read
========================================================================================


The tool aims to provide immediate access to SOTA models for scientific NLP.  My main concern with the paper is that the main claimed benefit with respect to other toolkits is that it provides access to SOTA models (with respect to those provided by other toolkits like AllenNLP, SciSpaCy, etc.)  But the paper doesn't include any empirical results to support this claim.  Also, I assume these are all moving targets as different toolkits incorporate new and better models.
----------------------------------------------------------------------------------------
Abhi: I agree in many cases they are not comparable. But in Citation intent classification we are 0.5 behind the state of the art without attention. I2B2 as well.
Addressed some of them in section 3.
==============================================================================================

---END----



==> SciWING - SDP/sections/conclusion.tex <==
\section{Conclusion and Future Work}

We introduce \sciwing{}, an open-source scholarly document processing (SDP) toolkit, targeted at practitioners and researchers interested in rapid experimentation.   It provisions pre-trained models for key SDP tasks 
% --- such as citation string parsing and citation intent classification ---
that achieve state-of-the-art performance and aids practitioners to deploy models directly on their community's literature.

\sciwing{}'s modular design also greatly facilitates SDP researchers in model architecture development, speeding train/test cycles for architecture search, and supporting transfer learning for use cases with limited annotated data. \sciwing{} allows declaration of models, datasets and experiment parameters in a single configuration file. 

\sciwing{} is actively being developed. We consider the following improvements in our roadmap:

\textbf{$\bullet$} \sciwing{} has yet to incorporate natural language generation related models. We would like to consider sequence to sequence neural models which have proven useful for scientific document summarization tasks, among others. 


\textbf{$\bullet$} Scientific document processing involves minimal training data and has found benefits in incorporating document structure, both of which are tackled using multi-task learning. Multi-task learning is thus a future milestone in \sciwing{}.

\textbf{$\bullet$} We would like \sciwing{} to foster collaboration among the SDP community and encourage assistance with these goals through contributions to our Github repository in the form of models, datasets and improvements to the framework.

% Our current development target is to incorporate models for sequence to sequence (seq2seq) generation which are useful for scientific document summarization, and multi-task learning (to ameliorate challenges with sparse data), alongside the implementation of additional SDP tasks and models.
% We hope that \sciwing{} fosters collaboration among the SDP community, and encourage assistance with these goals through contributions on our Github repository.

% Min: repo already mentioned at the beginning, the most useful place to put a URL.  No need to repeat.
% We are continuously developing tasks and models and the development can be tracked in the Github repository.



==> SciWING - SDP/sections/development_roadmap.tex <==
% Min: distributing this into your conclusion to save space.
% Currently this text is unused.
\section{Development Road Map}

\sciwing{} is developed actively. The project continues to add more models related to scientific document processing. We continue to support a wide range of transformers and other embeddings suitable for scientific document processing. Currently, \sciwing{} does not include models for sequence to sequence generation and we will be including it in the future releases of \sciwing{}. We also plan to include multi-task learning that has proven to be useful in scientific document processing that faces the challenge of small amounts of training data. 

==> SciWING - SDP/sections/introduction.tex <==
\section{Introduction}
Automated scientific document processing (SDP) deploys natural language processing (NLP) on scholarly articles.  As scholarly articles are long-form, complex documents with conventional structure and cross-reference to external resources, they require specialized treatment and have specialized tasks.  Representative SDP tasks include parsing embedded reference strings \cite{prasadanimesh,thai2020using}; identifying the importance, sentiment and provenance for citations \cite{Cohan2019Structural,Su2019NeuralML}; identifying logical sections and markup \cite{luong2012logical}; parsing of equations, figures and tables \cite{Clark2016PDFFigures2M}; and article summarization \cite{qazvinian-radev-2008-scientific,qazvininaradev2013,cohan-goharian-2015-scientific,cohan-etal-2018-discourse,cohanijdl}.  SDP tasks, in turn, help downstream systems and assist scholars in finding relevant documents and manage their knowledge discovery and utilization workflows. 
Next-generation introspective digital libraries such as Semantic~Scholar~\cite{ammar-etal-2018-construction}, Google Scholar and Microsoft Academic have begun to incorporate such services. 

\begin{figure}[t!]
    \centering
    % Min: like the other diagram, this figure needs to be more readable.  The font selection and and dark on light won't work well for printout.  Consider black on light grey and using a smaller set of font sizes.  
    % Min: the architecture terminology needs also to fit the text.  Models, Modules, Modelling, Engine, Framework are all confused terminology.  See text.
    % Min2: formatting in the caption seems off.  You have some bolded, some italicized.  Be consistent.
    %Abhi2: Fixed this
    \includegraphics[width=0.5\textwidth]{images/sciwing_arch_new.png}
    % Min2: really hard to read the small text.  Consider using the reverse gradient coloring, using higher contrast blocks for the small models and darker ones at the top.
    \caption{\sciwing{} Components: Text classification 
    % Min2: what's Clf?  Instead use a smaller font or less of a l/r cell padding 
    % Min2: consider moving SciWING logo into the bottom right or left to save vertical space in the image
    % Min2: check my edit.
    % Abhi2: Removed the shortforms. Changed the image to svg for better clarity. The readability must be better now.
     and Sequence labelling {\bf Datasets}, {\bf Models} composed from low-level {\bf Modules}, and \textbf {Engine} to train and record experiment parameters. {\bf Infer} middleware does the inference and high-level functionality (e.g., developing APIs; low-level and web applications).}
    \label{fig:sciwing_arch}
\end{figure}

\begin{table*}[t!]
    \centering
    \begin{tabular}{c c c c c c}
    \textbf{Framework} & \textbf{Pre-trained models} & \textbf{SOTA} &\textbf{ Neural first} & \textbf{Extensible} & \textbf{Language/Framework} \\
    \hline
    SciSpaCy & \greencheckmark &  & & & Py \\ 
    AllenNLP & \greencheckmark & & \greencheckmark & \greencheckmark & Py(Torch) \\ 
    \textsc{flair} & \greencheckmark & & \greencheckmark & \greencheckmark & Py(Torch) \\
    Grobid &  \greencheckmark & & & & Java \\ 
    \hline 
    \sciwing{} & \greencheckmark & \greencheckmark & \greencheckmark & \greencheckmark & Py(Torch) \\ 
    \hline
    \end{tabular}
    % Min2: Takes up a lot of space.  Useful to have a grid comparison but not sure it is so worth the space.  Can you make it 1-col with less captions?  
    % Min2: is SciSpacy an SDP framework?  What do you mean by ``other NLP frameworks''?
    % Abhi2: Brought this back in to improve space utilization and improve readability.
    \caption{Comparison of \sciwing{} with popular frameworks. \textbf{Pre-trained models}: availability of pretrained models. \textbf{SOTA}: state-of-the-art or comparably performing models for SDP. \textbf{Neural-Networks first}: supports end-to-end neural network development and training. \textbf{Extensible}: easily incorporates new datasets and architectures.}
    \label{tab:framework-comparison}
\end{table*}

While NLP, in general, has seen tremendous progress with the introduction of neural network architectures and general toolkits and datasets to leverage them, their deployment for SDP is still limited.  Over the past few years, many open-source software packages have accelerated the development of state-of-the-art (SOTA) NLP models. However, these frameworks have a few limitations concerning SDP. First, most are general purpose frameworks aimed at producing SOTA models for natural language understanding tasks or only for specific domains such as biomedicine. Second, they do not provide deployable, SOTA models for SDP. Most provide limited or no means for researchers to train models on their datasets, or experiment with model architectures.

% Hugging Face's transformer models \cite{Wolf2019HuggingFacesTS} and AllenNLP \cite{Gardner2017AllenNLP} are general-purpose frameworks that have produced state-of-the-art models for natural language understanding tasks. 
% SciSpacy \cite{Neumann2019ScispaCyFA} is a non neural network based pipeline for biomedical documents related tasks and does not facilitate training alternate models on other datasets. Grobid \cite{GROBID} is the closest to our work. However, it is not a neural-network first framework and is not preloaded with SOTA models.

% \begin{table}[t!]
%     \centering
%     \small
%     \begin{tabular}{|c|c c c c|c|}
%     \hline
%     Framework & P & S & N & X & Language\\
%     \hline
%     SciSpacy & \greencheckmark &  & & & Python \\ 
%     AllenNLP & \greencheckmark & & \greencheckmark & \greencheckmark & Py(Torch) \\ 
%     Grobid &  \greencheckmark & & & & Java \\ 
%     SciWING & \greencheckmark & \greencheckmark & \greencheckmark & \greencheckmark & Py(Torch) \\ 
%     \hline
%     \end{tabular}
%     % Min2: Takes up a lot of space.  Useful to have a grid comparison but not sure it is so worth the space.  Can you make it 1-col with less captions?  
%     % Min2: is SciSpacy an SDP framework?  What do you mean by ``other NLP frameworks''?
%     % Abhi2: This has been resolved
%     \caption{Comparison of SDP frameworks. P, S, N, X denote (P)retrained models, (S)tate-of-the-art performance, (N)eural-first models, and e(X)tensibility.}
%     \label{tab:framework-comparison}
% \end{table}

A key barrier to entry is accessibility: a non-trivial level of expertise in NLP and machine learning is a prerequisite.  Practitioners who wish to deploy SDP on their field's literature may lack knowledge and motivation to learn it for the sake of deployment.  Thus, there is a clear need for a toolkit that unifies different efforts and  provides access to pre-trained, SOTA models for SDP, while also allowing researchers to experiment with models rapidly to create deployable applications.

We introduce \sciwing{} to address this need with respect to other frameworks (cf. Table~\ref{tab:framework-comparison}). Built on top of PyTorch, 
% Min2: doesn't add much, removed.
%and under active development
it provides access to neural network models 
% MinCR: can we say pre-trained
% trained 
%AbhiCR: Changed it 
pre-trained
for a growing number of SDP tasks which practitioners can easily deploy on their documents.
For researchers, these models serve as baselines and \sciwing{} encourage them to try architectural variations in a modular manner by swapping or composing 
% different neural network 
modules 
% MinCR: rephrased
in a declarative manner in a configuration file, 
without having to program or deal with complexities of generic tools like AllenNLP \cite{Gardner2017AllenNLP}. 
% \sciwing{} also allows researchers to declare models in a configuration file without having to write programming code.


\sciwing{} is MIT licensed and comes with downloadabled pre-trained models and freely-available datasets. The package runs on Python 3.7 and can be easily installed from Python Packaging Index (PyPI) using \texttt{pip install sciwing}. For researchers aiming to further develop \sciwing{}, we provide installation tools that set up the system, alongside 
% Min2: I think `extensive' is a stretch :D :D
% extensive 
documentation. 
% Min2: not sure this adds anything. Omitted
% We envision that \sciwing{} will make scientific document processing more accessible and facilitates easy experimentation with neural network model architectures.  

% Min: distribute this to system_overview.
% \sciwing{} incorporates AllenNLP \cite{Gardner2017AllenNLP} and develops models on top of it and uses the transformers package to enable transfer learning using pre-trained general-purpose transformers such as BERT \cite{devlin-etal-2019-bert} and SDP-specific ones; i.e., SciBERT \cite{Beltagy2019SciBERT}. 

% Min: I think this list is pretty redundant with your intro written as is already.  I suggest you save the space for more meaningful information.  
%\sciwing{} embraces the following core principles:

%\begin{itemize}
%    \item \textbf{Ease of Use} - \sciwing{} should allow practitioners to get predictions from state-of-the-art models for their own data. It should provide an eco-system for researchers to experiment in a reproducible manner, and allow easy logging of experiment artefacts. 
    
%    \item \textbf{State of the art models} -\sciwing{} should provide out-of-the-box access to state-of-the-art models for scientific document processing.
    
%    \item \textbf{Modularity} - \sciwing{} should enable easy construction of neural network architectures in a modular manner. 
    
%    \item \textbf{Flexibility} - \sciwing{} should allow researchers to have access to pre-trained neural networks models for scientific document processing to begin with and experiment by swapping different pre-trained embeddings and transformers that are suitable for scientific document processing. Researchers should be enabled to perform experimentation with various deep learning hyper-parameters. 

%    \item \textbf{Open Source} - \sciwing{} should be open source and foster collaboration in the research community 
% \end{itemize}

% Min: still needed?  Distributed parts into the other parts of the intro.
% Driven by these principles, we have developed \sciwing{} \footnote{https://github.com/abhinavkashyap/sciwing}. 
% It is under active development with easy access to state-of-the-art models for many scientific document processing tasks. 
% We plan to release many more pre-trained models for scientific document processing. 

==> SciWING - SDP/sections/related_work.tex <==
\section{Related Work}
\label{sec:related-work}
Grobid~\cite{GROBID} is the closest to a general workbench for scientific document processing. 
Similarly to \sciwing{}, Grobid also performs document structure classification, reference string parsing, among other tasks. But Grobid is architected in the traditional, manual feature engineering approach, leading to performance losses for many SDP tasks, and difficulties in retrofitting neural models into its framework.   

SciSpaCy~\cite{Neumann2019ScispaCyFA} focuses on biomedical related tasks such as POS-tagging, syntactic parsing and biomedical span extraction.  However, SciSpaCy primarily caters for practitioners; it does not easily allow for the development and testing of new models and architectures.  

% BUG Min: overly repetitive with intro.  Edit down the redundancy here or in the other section.  Too wordy.
% FIXED: Abhi
Task- and domain-agnostic frameworks also exist.  NCRF++ \cite{yang2018ncrf} is a tool for performing sequence tagging using Neural Networks and Conditional Random Fields and \textsc{flair} \cite{akbik2018coling} is a framework for general-purpose NLP and mainly provide access to different embeddings and ways to combine them.

% \sciwing{} interfaces with general purpose AllenNLP framework~\cite{Gardner2017AllenNLP} and transformers framework \cite{Wolf2019HuggingFacesTS} for pre-trained transformer architectures such as ELMo, BERT, SciBERT, etc.
% Min2: Still repetitive.
% Abhi2: Removed this. And mentioned that we use AllenNLP and HuggingFace transformers for contextual word representations.
% \sciwing{} builds on top of it to give researchers easy access to general-purpose and SDP-specific contextual word embeddings.


==> SciWING - SDP/sections/system_overview.tex <==
%\sciwing{} 
\section{System Overview}

Our view is that SDP-specific considerations are best embodied as an abstraction layer over existing NLP frameworks.  \sciwing{} incorporates AllenNLP, the generic NLP pipeline \cite{Gardner2017AllenNLP}, developing models on top of it when necessary, while using the transformers package \cite{Wolf2019HuggingFacesTS} to enable transfer learning via its pre-trained general-purpose representations such as BERT \cite{devlin-etal-2019-bert} and SDP-specific ones like SciBERT \cite{beltagy-etal-2019-scibert}. 
Fig.~\ref{fig:sciwing_arch} shows 
\sciwing{}'s Dataset, Model and Engine components facilitating flexible re-configuration.  We now describe these components.

% \sciwing{} builds with Python 3.7 and is provisioned as a package available on the Python Packaging Index (PyPI), supporting installation via \texttt{pip install sciwing}.  This downloads its PyTorch and other library dependencies. For users aiming to develop the library further, \sciwing{} comes with installation tools that set up the system, alongside extensive in-lined code documentation, and explanatory tutorials.

% Min2: maybe use the same bulleting environment as in Section 3 that outdents the bullets.  Saves space (marginally) while preserving consistent formatting.
% Abhi2: This has been changed

    \vspace{2mm}
    \textbf{Datasets}: There are many challenges for the researcher--practitioner to experiment with different SDP tasks.  First, 
    % MinCR: simplify
    % researchers are often dealt with the challenge of handling various formats of the datasets
    researchers must handle various data formats and datasets: for reference string parsing, the CoNLL format is most common; for text classification, CSV is most common. \sciwing{} enables reading of dataset files in different formats and also facilitates the download of open datasets using command-line interfaces. For example, \texttt{sciwing download data --task scienceie} downloads the official, openly-available dataset for the ScienceIE task.  
    
    Current methods for pre-processing are cumbersome and error-prone.  Processing can become complex when different models require different tokenisation and numericalisation methods.  \sciwing{} unifies these various input formats through a pipeline of pre-processing, tokenisation and numericalisation, via \texttt{Tokenisers} and \texttt{Numericalisers}. \sciwing{} also handles batching and padding of examples.
    \vspace{1mm}
    
    % Min2: can't parse.  Does this mean the subcomponents are pytorch classes?
    % Abhi2: Everything here are Pytorch classes
    \textbf{Models}: Paired Embedder--Encoder subcomponents combine to form a neural network model, themselves PyTorch classes. 
    
    % \textbf{$\bullet$ Embedders}: 
    {\it Embedders}: Modern NLP models represent natural language tokens as continuous vectors -- embeddings.  \sciwing{} abstracts this concept via \texttt{Embedders}.  Generic (non-SDP specific) embeddings such as GlovE \cite{pennington-etal-2014-glove} are natively provided.  Tokens in scientific documents can benefit from special attention, as most are missing from pre-trained embeddings. \sciwing{} includes task-specific trained embeddings for reference strings \cite{prasadanimesh}. \sciwing{} also supports contextual word embeddings: ELMo~\cite{peters-etal-2018-deep}, BERT~\cite{devlin-etal-2019-bert}, SciBERT~\cite{beltagy-etal-2019-scibert}, etc. SOTA embedding models are built by concatenating multiple representations, via \sciwing{}'s \texttt{ConcatEmbedders} module. As an example, word and character embeddings are combined in NER models~\cite{lample-etal-2016-neural}, and multiple contextual word embeddings are combined in various clinical and BioNLP tasks \cite{zhai-etal-2019-improving}.
    
    % \textbf{$\bullet$ Neural Network Encoders}: 
    {\it Neural Network Encoders}: \sciwing{} ports commonly-used neural network components that can be composed to form neural architectures for different tasks. For example in text classification, encoding input sentence as a vector using an LSTM is a common task 
    (\sciwing{}'s 
    \texttt{seq2vecencoder}). Another common operation is obtaining a sequence of hidden states for a set of tokens, often used in sequence labelling tasks and 
    \sciwing{}'s 
    \texttt{Lstm2seq} achieves this. Further, it also includes attention based modules.
    
    \sciwing{} builds in generic linear classification and sequence labelling with CRF heads that can be attached to the encoders to build production models. It provides pretrained SOTA models for particular SDP tasks that work out-of-the-box 
    % for prediction 
    or further fine-tuned.  
    
    % Min: best described in the tasks/dataset section
    % The \texttt{NeuralParsCit} model for the reference string parsing task is such an example, consisting of a concatenation of word, character and ELMo embeddings and a Bidirectional-LSTM with CRF layer \cite{lample-etal-2016-neural}. 
    \vspace{2mm}
    
    \textbf{Engine}: 
    \sciwing{} handles all the boilerplate code to train the model, monitor the loss and metrics, check-pointing parameters at different stages of training, validation and testing. It helps researchers adopt best practices, such as clipping gradient-norms, as well as saving and deploying best performing models. 
    % MinCR: both clauses redundant
    % AbhiCR: Needs no action 
    % \sciwing{}'s experimentation framework is flexible and users have the flexibility of customizing the following:
    % \sciwing{}
    Users can customize the following: \\

    % \textbf{$\bullet$ Optimisers}: 
    {\it Optimisers}: \sciwing{} supports all the optimisers supported by PyTorch, and various learning rate schedulers that dynamically manage learning rates based on validation performance.
    
    % \textbf{$\bullet$ Experiment Logging}: 
    % Min2: rewriting this section.  Please check.
    % Logging the hyper-parameters of the model is a tedious task. However, many online logging tools have alleviated the difficulty of managing experiments. \sciwing{}  writes logs for every experiment run and also facilitates cloud-based experiment logging and corresponding charting of relevant metrics. via the third-party API service of {\it Weights and Biases} \url{www.wandb.com}.  Integrating alternative services for experiment logging is work-in-progress. 
    % Abhi2: This looks okay
    {\it Experiment Logging}:
    \sciwing{} adopts current best practices in leveraging logging tools to monitor and manage experiments. \sciwing{} writes logs for every experiment run and facilitates cloud-based experiment logging and corresponding charting of relevant metrics via the third-party API service of {\it Weights and Biases}\footnote{\url{www.wandb.com}.}, with the integration of alternative logging services on the way.
    
    % \textbf{$\bullet$ Metrics}: 
    {\it Metrics}: Different SDP tasks require their respective metrics. \sciwing{} abstracts a separate \texttt{Metrics} module to select appropriate metrics for each task. \sciwing{} includes \texttt{PrecisionRecallFMeasure} suitable for text classification tasks,  \texttt{TokenClassificationAccuracy}, and the official CONLL2003 shared task evaluation metric
    % MinCR: implied. not needed 
    %AbhiCR: No action needed
    % \footnote{Based on the official $conlleval$ script from CoNLL.}
    suitable for sequence labelling. \\
    
\noindent With these components given, \sciwing{}'s \textbf{Inference} middleware provides clear abstractions to perform inference once models are trained. The layer runs predictions on the test dataset, user inputs and files.  Such abstractions also act as an interface for the development of upstream REST APIs and command-line applications. 
    
\subsection{Configuration using TOML} 

\sciwing{}'s flexible architecture is encapsulated by its use of declarative TOML configuration files.  TOML was chosen as it is a widely-used, unambiguous, and human-readable configuration file format.
This enables users to declare dataset, model architectures and experiment hyper-parameters in a single place. \sciwing{} parses the TOML file and creates appropriate instances of the dataset, model and engine to run experiments.

A simple configuration file for reference string parsing  along with its equivalent model declaration in Python is shown in the listings below. The class declaration % in Python 
and configuration file have a one-to-one correspondence.  As deep learning models are made of multiple modules, \sciwing{} % adopts a strategy to
automatically instantiates these submodules as needed. \sciwing{} constructs a Directed Acyclic Graph (DAG) from the model definition to achieve this. The DAG's topological ordering instantiates the different submodules to form the final model.\\

\begin{lstlisting}[language=XML, basicstyle=\small]
[model]
    class="SimpleClassifier"
    encoding_dimension=300
    num_classes=23
    classification_layer_bias=true
    [model.encoder]
        emb_dim=300
        class="BOW_Encoder"
        dropout_value=0.5
        aggregation_type="sum"
        [[model.encoder.embedder]]
        class="VanillaEmbedder"
        embed="word_vocab"
        freeze=False
\end{lstlisting}

\begin{lstlisting}[language=Python, basicstyle=\small]
class SimpleClassifier(nn.Module):
    def __init__(
    self, 
    encoder: nn.Module,
    encoding_dim: int,
    num_classes: int,
    classification_layer_bias: bool)
\end{lstlisting}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/toml_vs_python.png}
%     \caption{(l) The model section of the TOML file, and (r) its corresponding class declaration in Python.}
%     \label{fig:tomlvpython}
%     % Min2: still too small.  Consider putting in the lstlisting environment to be consistent across the paper.
%     % Abhi2: Has been changed to two lstlistings code.
% \end{figure}

\subsection{Command Line Interface}
\label{sec:command-line-interfaces}
Qualitatively analyzing the results of the model by drilling down to certain training and development instances can be telling and help to diagnose performance issues. \sciwing{} facilitates this by providing an interactive inspection of the model  through a command-line interface (CLI). Consider the task of reference string parsing: the confusion matrix for the different classes can be displayed through the provided CLI utility, which also allows finer-grained introspection of (Precision, Recall, F-measure) metrics and the viewing of error instances where one class is confused for another. For example, \texttt{sciwing interact neural-parscit} provides introspection utilities for the pre-trained reference string parsing model. Such introspection utilities are also available for other pre-trained models.

\sciwing{} provides commands to run experiments from the configuration file, aiding replication. For example, experiments declared in a file named \texttt{experiment.toml}, can be run with the command \texttt{sciwing run experiment.toml}. \sciwing{} then saves the best model. \texttt{sciwing test experiment.toml} invokes inference which deploys the best model against the test dataset and displays the resultant metrics.

\subsection{End User Interfaces}
\sciwing's API service enables the development of various graphical user interfaces. \sciwing{} uses its \textit{Infer} layer and exposes APIs for various tasks including reference string parsing, citation intent classification, extracting abstracts and logical sections of articles, identifying entities in clinical notes, using \texttt{fastapi}\footnote{https://fastapi.tiangolo.com/}.
% BUG Min: can you list the APIs that are implemented?  Perhaps in the use case on NPC, go through all of the interfaces that enable all of us.
% We have the ParsCit API and I am developing the one for citation intent classification now (Supposed to be done by Ding Xu. I have not received any update for him)
% FIXED: Abhi
The API enables the following application families downstream:\\
% Min2: maybe use the same bulleting environment as in Section 3 that outdents the bullets.  Saves space (marginally) while preserving consistent formatting.
% Abhi2: Is now the same everywhere

     \textbf{$\bullet$ Web Demonstrations}: To provide quick access to predictions from state-of-the-art models, fulfilling one key aim of \sciwing{}, we have developed an interactive demo using streamlit\footnote{http://www.streamlit.io}:  \url{http://rebrand.ly/sciwing-demo}. Pre-specified data or user data can be  processed using the distributed models (Figure~\ref{fig:parscit-demo}). Both API services and demos can also be run by installing \sciwing{} locally.
    
    \textbf{$\bullet$ Programmatic Interfaces} in \sciwing{} provisions advanced use. Users can make predictions for documents stored as .pdf or text files. For example, to parse a text file's citations, \sciwing provides a \texttt{NeuralParscit} class that has methods to parse all the strings in a file, storing them in a new file. Such a programmatic interface helps the practitioner make predictions easily.

\begin{figure*}
    \centering
    % \includegraphics[width=0.5\textwidth]{images/parscit_web_demo.png}
    \includegraphics[width=\textwidth]{images/parscit_web_demo_sideways.png}
    % BUG Min: Neural Parscit => Neural ParsCit (use correct casing) in your screenshot - i.e., change the string in the web demo 
    % BUG Min: text too small.
    % BUG Min2: fix your captions footnotes.  Some redundant with previous mentions.
    % FIXED: Apparently we have to write footnotes manually and manage the numbers manually as well. Just putting the information within the caption itself
    \caption[]{Sample \sciwing{}'s demonstration (\url{https://rebrand.ly/sciwing-demo}) for reference string parsing model, where input (l) is then classified into 13 output classes (r). We utilize the displaCy visualization toolkit (www.spacy.io) and  streamlit (www.streamlit.io).  }
    \label{fig:parscit-demo}
\end{figure*}

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l | c | c}
        \hline
         \textbf{Task} & \textbf{SciWING} & \textbf{Best} \\
         \hline 
         Reference String Parsing & \textbf{88.44} & --- \\
         % Min2: BUG missing numbers
         % Fixed: Abhi
         ScienceIE & \textbf{49.9} & 48.01 \\ 
         Logical Structure Recovery & \textbf{73.2} & --- \\ 
         Citation Intent Classification & 82.16  & 82.6 \\ 
         I2B2 NER & 85.83 & 86.23 \\
         \hline 
    \end{tabular}
    \caption{\sciwing{}'s SDP task performance, compared against other comparable models. 
    % MinCR: added see whether ok with you.
    %AbhiCR: I added it initially and had my doubts. But, it is okay.
    Bolded values indicate state-of-the-art or comparable performance (without attention).
    % 
    Scores are macro $F_1$.}
    % Min2: this table not referenced anywhere.
    % MinCR: Table looks weird not the regular Table format.
    % AbhiCR: Just keeping this style of the table for now
    % Abhi: Has been fixed by Min
    % MinCR: Put all of these as bold if they are actually comparable, or drop the SOTA checkmark in the table.  I've already changed the table to say it's comparable in the other table. 
    % AbhiCR: The bolds are true. We can claim SOTA on them.
    \label{tab:sdp_performance}
\end{table}

\section{Tasks}
\sciwing{} prepackages models for various SDP tasks.  The examples demonstrate how to use the framework effectively. These models have performance close or comparable to state-of-the-art models (Table~\ref{tab:sdp_performance}).  They are production-ready, but also can be used as baselines for further research.\\

    \textbf{$\bullet$ Reference String Parsing} assigns one of 13 classes to tokens of a reference string that correspond with a in-document citation: {\it author}, {\it journal} and {\it year} of publication, among them.  Neural sequence labelling models, combining a bidirectional LSTM with CRF currently yield top results \cite{prasadanimesh}. The model included in \sciwing{} implements the same model architecture, but adds ELMo embeddings.  Unfortunately, due to the high training expense of their 10-fold cross validation, we are not able to obtain directly comparable results to their model's performance.

    \textbf{$\bullet$ ScienceIE} identifies typed keyphrases, originally from chemical documents: {\it Task} keyphrases that denote the end task or goal, {\it Material} keyphrases indicate any chemical, and {\it Dataset} that is being used by the scientific work and the process includes any scientific model or algorithm.
    % Min: cite the work
    % Abhinav: Done
    The state-of-the-art system from 2017 includes a word and character embeddings and a bidirectional LSTM with CRF and uses language model (LM) embeddings \cite{ammar-etal-2017-ai2}. \sciwing{} includes a reference implementation without using LM embeddings and the results are comparable. We use the same dataset used by \cite{luong2012logical} for training the neural networks.

    \textbf{$\bullet$ Logical Structure Recovery} identifies the logical sections of a document: introduction, related work, methodology, and experiments.  This drives the relevant, targeted text to downstream tasks such as summarization, citation intent classification, among others. Currently, there are no neural network methods for this task, so \sciwing{}'s models can serve as strong baselines.

    \textbf{$\bullet$ Citation Intent Classification} identifies the purpose of a citation. Some citations refer to another work for {\it background} knowledge, a few to a related work's {\it results} and others to {\it compare and contrast} their methods or results. Such citation intents get used in Semantic Scholar\footnote{www.semanticscholar.org}. We train a
    % bidirectional LSTM with Elmo on the Scicite dataset 
    bi-LSTM with ELMo on the Scicite dataset and achieve an F-score of 82.16. \cite{Cohan2019Structural} use Bi-LSTM with attention   At the time of writing, \sciwing \ does not include attention models, and as such results are not strictly comparable. We plan to include attention-based models in future iterations of the package.
    
    \textbf{$\bullet$ I2B2 Named Entity Recognition} identifies three kinds of entities from clinical notes; problems (e.g., a disease), treatments (e.g., a drug) and tests (e.g., diagnostic procedures). We use a similar model of Bi-LSTM CRF with ELMo embeddings, achieving 85.83 $F_1$. 
 
% Min2: Vacuous.  Omitting   
%    Other tasks and datasets are being actively developed.  We envision the development of additional models will be swift and easy.

%% Min: end import from tasks.
%    \vspace{2mm}
    


==> SciWING - SDP/sections/tasks.tex <==
% \section{Example Tasks}
% \sciwing{} includes examples for various task  which finds wide-spread use in scientific document processing. The examples demonstrate how to use the framework effectively. The models have verified performance levels that closely match the performance of the original results. They can be used as baselines for further research.

\begin{itemize}
    \item \textbf{Logical Structure Recovery} - Identifying the different logical sections of a research article like the introduction, conclusion, methodology experiments and others can aid in many downstream task like summarization, citation intent classification amongst others. Currently there are no neural network methods for logical structure recovery. We use the same dataset as \cite{kan}
    Examples neural network models which can serve as baselines for future research are included in \sciwing{}. 
    \textbf{\item Citation String Parsing} - Citation string parsing identifies the different parts of a citation string like the author of the research article, the journal and the year of publication and other data. Neural network methods for citation string parsing has shown good promise \cite{prasadanimesh}.  Citation string parsing is a sequence labelling task and \cite{prasadanimesh} combines a bidirectional LSTM with CRF. \sciwing{} includes the same architecture but also combines with ELMo embeddings.
    \textbf{\item ScienceIE task} - The task is to identify the different key-phrases in a scientific document. There are three key-phrases to be identified. Task key-phrases that denote the end task or goal, the material key-phrases indicate any chemical, dataset that is being used by the scientific work and the process includes any scientific model or algorithm. The state of the art system from 2017 includes a bidirectional LSTM with CRF and uses language model embeddings. \sciwing{} includes a reference implementation for the model but uses ELMo embeddings instead of the language model representations.
\end{itemize}

Other models are being actively developed for scientific document processing. We expect, that the development of these models is swift and easy and steadily grows over time.  The example implementations of these models can be found at \url{https://github.com/abhinavkashyap/sciwing/examples}.

==> SciWING - SDP/sections/use_case.tex <==
\section{Use Cases}

\sciwing{} caters to both use cases of practitioners looking to deploy pre-trained models as well as researchers looking to refine model architectures and perform fine-tuning domain adaptation on top of state-of-the-art contextual word embedding models.  We now examine both use cases.

\subsection{Using Pre-trained Reference String Parser}
\sciwing{} provisions out-of-the-box access to pretrained models for direct deployment. Citation string parsing can be deployed with just a few lines of code as shown below.

% Min2: runs over left margin.  Fix
% https://tex.stackexchange.com/questions/83614/set-horizontal-width-on-custom-listings-environment
\begin{lstlisting}[language=Python, basicstyle=\small]
from sciwing.models.neural_parscit import NeuralParscit

# instantiate the best model for reference string parsing.
neural_parscit = NeuralParscit()

# predict for some reference
neural_parscit.predict_for_text("reference")

# predict for a file containing one reference per line 
neural_parscit.predict_for_file(/path/to/file)
\end{lstlisting}

% Behind the scenes, 
% Min2: repetitive with earlier sections.
% Abhi2: Moved to the previous section.
% \sciwing{} instantiates the best neural network architecture and downloads the best weights from our web-servers. We also provide introspection utilities to inspect the results of the best model on the test dataset. \texttt{sciwing inspect neural-parscit} enables to see the confusion matrix, see examples of instances which are misclassified, inspect the precision, recall and F-measure on the test set, enter text to get the results. 

\subsection{Building a Reference String Parser from Scratch}

State-of-the-art models can be built by stacking up multiple components. We illustrate how to construct such \sciwing{} models, building up to such SOTA model by simple modifications. Such step-by-step model creation also facilitates ablation studies, a common part of empirical studies.
\vspace{1mm}

\textbf{1. Bi-LSTM tagger}:
Our base model is a bi-LSTM with a  GLoVE embedder.  Every input token is classified into one of 13 different classes.
\begin{lstlisting}[language=Python, basicstyle=\small]
# initialize a word embedder 
word_embedder = WordEmbedder(
    embedding_type = "glove_6B_100")

# initialize a LSTM2Seq encoder
lstm2seqencoder = LSTM2SeqEncoder(
    embedder = word_embedder, 
    hidden_dim = 100,
    bidirectional = True)

# initialize a tagger without CRF
model = SimpleTagger(
    rnn2seqencoder = lstm2seqencoder, encoding_dim = 200)
\end{lstlisting}

\textbf{2. Bi-LSTM Tagger with CRF}:
We then make a single modification to the above code, swapping the simple tagger with one that uses a CRF.
\begin{lstlisting}[language=Python, basicstyle=\small]
...

# an RNN tagger with CRF on top
model = RnnSeqCrfTagger(
    rnn2seqencoder = lstm2seqencoder, encoding_dim = 200
)
\end{lstlisting}

\textbf{3. Bi-LSTM tagger with character and ELMo Embeddings}:
We modify the code to include a bidirectional LSTM character embedder.  We use the ConcatEmbedders module to create the final word embeddings (Line~16), which concatenates the character embeddings with those from the previous word embedding and a pretrained ELMo contextual word embedding. 
This final model is the provisioned model for the reference string parsing task provided in \sciwing{}.

\begin{lstlisting}[language=Python, basicstyle=\small]
...
word_embedder = WordEmbedder(
   embedding_type = "glove_6B_100"
)

# LSTM character embedder
char_embedder = CharEmbedder(
   char_embedding_dimension = 10,
   hidden_dimension = 25,
)

# ELMo embedder
elmo_embedder = ElmoEmbedder()

# Concatenate the embeddings
embedder = ConcatEmbedders([word_embedder, char_embedder, elmo_embedder])
\end{lstlisting}

Here we have described one use case, but models for other tasks are built as easily. In a similar way, we have built a similar architecture for the clinical notes parsing task --- the ScienceIE task I2B2 NER task.

==> comments/comments.emnlpdemo.tex <==
Dear Abhinav Ramesh Kashyap:

I am sorry to inform you that the following submission was not selected by the program committee to appear at EMNLP - Demonstrations 2020:

SciWING - A Software Toolkit for Scientific Document Processing

The selection process was very competitive. Due to time and space limitations, we could only choose a small number of the submitted papers to appear on the program. Nonetheless, I still hope you can attend the conference.

I have enclosed the reviewer comments for your perusal.

If you have any additional questions, please feel free to get in touch.

Best Regards,
David Schlangen and Qun Liu
EMNLP - Demonstrations 2020

============================================================================ 
EMNLP - Demonstrations 2020 Reviews for Submission #83
============================================================================ 

Title: SciWING - A Software Toolkit for Scientific Document Processing
Authors: Abhinav Ramesh Kashyap and Min-Yen Kan


============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 4
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 5
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper describes a toolkit for scientific document processing. It allows several NLP tasks such as reference string parsing, scienceIE, and I2B2 NER. It provides CLI, Python, and Web API.

STRENGTHS:
1. The software is easy to use (can be installed using pip) with lots of examples. It provides many interfaces and can be customized/extended easily.
2. The demo site (which is different from the one written in this paper) vividly shows how this toolkit can be used to perform scientific document processing.
3. It contains up-to-date pre-trained models and is actively maintained.

WEAKNESSES:
1. The development of the software is mainly done by a single person (the first author of this paper). It would be great if the software can be maintained by a group of people (it is often the case that software will become unmaintained after the initial release if the person lost his interest/becomes busy/etc.). 
2. (probably related to the previous point) It is hard to keep the environment up-to-date. It is better to "freeze" the versions of deep learning toolkits and libraries because otherwise "pip install" often breaks (From my experience, I have to update the versions of CUDA and PyTorch every year unless I pin down the versions, otherwise the software won't work as expected). 
https://github.com/abhinavkashyap/sciwing/issues/22

Style:
The code snippet in this paper looks a bit strange. I would suggest using a different font.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 3
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 1
                    Recommendation (1-5): 3
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper presents SciWING, a platform that supports SDP tasks. One of the main goals is to provide a flexible framework to support SDP tasks for non-NLP experts by providing pre-trained models for scientific data. The authors compare with existing frameworks and present a clear motivation for the work. They show how to configure the system, and discuss several related tasks.

Strength:

- The authors did extensive work on the SciWING APIs
- The technical description of the system and how to use it is well detailed and explained

Weaknesses:

- The authors claim that the platform is for non-NLP experts that wish to do some research on Scientific data. Given this, does your system provide suggestions or recommendations of what components are "making sense" to use during the building part?
- Some details and choices are not entirely clear:
o For the Logical Structure recovery task - how it was trained, which data was used?
o although the authors mention in the future work the task of Summarization (as part of generation), it seems to be one of the important and recent tasks comparing for example with niche tasks such as citation intent classification. Thus it is not clear what was the criteria for the chosen tasks.
- In order to fully understand the platform capabilities, it would be nice to show how general is the system by, for example, showing for NER is also perform on different datasets such as BC5CDR or NCBI-disease.
- Although a demo link was provided it was not accessible (during several different times that I've checked)
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 2
      Originality / Innovativeness (1-5): 3
                 Technical Quality (1-5): 3
        Impact of Ideas or Results (1-5): 3
Effectiveness of the Screencast video (1-5): 3
                    Recommendation (1-5): 2
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
This paper presents a tool for scientific document processing.  While this is an important and somewhat understudied problem domain, I feel like the paper makes claims that are unsubstantiated or inadequately defined, and it also does not sufficiently clarify its unique contributions over existing work. While the idea of a user-friendly and state-of-the-art scientific document processing library is perhaps a worthy goal, SciWING may need further refinement before it is ready to be presented as a demo at EMNLP.

Table 1 is very important -- it makes strong claims about the advantages of SciWING over existing toolkits.  Thus, it’s problematic that the columns of that table (corresponding to qualities that the paper claims SciWING has and previous toolkits lack) are not defined in the paper.  What does “neural-first” mean, in terms of what one can do with the toolkit?  What qualifies as “extensible”?  What workload do the authors use to claim that their approach is “SOTA” and none of the others are?

I was also not clear on what SciWING offers that differs from the base capabilities in AllenNLP.  Most of what the paper mentions in Section 2 -- the models, the training and testing capability, tokenizers, logging, metrics, support for embeddings, seem like AllenNLP components.  The TOML configuration file seems like an analogue to AllenNLP configuration files, albeit in a slightly different format.  Taking capabilities from AllenNLP makes perfect sense -- but the paper needs to be much more clear on what capabilities are new in this tool, versus built-in to AllenNLP.

Finally, related to my question about Table 1, I also found it confusing that the paper refers to itself as “SOTA” and all other tools as “not SOTA”, given that SciWING underperforms the state of the art in three of the four tasks where a comparison is made in Table 2.  Some of these performance gaps seem practically significant (e.g., the 2% absolute increase in reference parsing error seems like it would drive practitioners to use another tool instead -- can the authors bring this number up by incorporating other approaches?).
---------------------------------------------------------------------------




==> comments/comments.sdp.tex <==
============================================================================ 
SDP 2020 Reviews for Submission #17
============================================================================ 

Title: SciWING– A Software Toolkit for Scientific Document Processing
Authors: Min-Yen Kan and Abhinav Ramesh Kashyap


============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 2
           Soundness / Correctness (1-5): 4
             Meaningful Comparison (1-5): 2
                      Thoroughness (1-5): 2
        Impact of Ideas or Results (1-5): 3
                    Recommendation (1-5): 3
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
The paper presents SYS, an open source toolkit that packages existing models for scientific document processing.  The toolkit provides access to both a command-line interface and a web interface.

The tool aims to provide immediate access to SOTA models for scientific NLP.  My main concern with the paper is that the main claimed benefit with respect to other toolkits is that it provides access to SOTA models (with respect to those provided by other toolkits like AllenNLP, SciSpaCy, etc.)  But the paper doesn't include any empirical results to support this claim.  Also, I assume these are all moving targets as different toolkits incorporate new and better models.

In any event, I do think there is some value in having more innovation in toolkits that provide easy access to NLP models, so there is some merit to this work.  This is a more like a demo paper than a traditional workshop paper presenting new empirical results, but I do think it fits the theme of the workshop.

One other concern: the paper does include links to the toolkit and demo that break anonymity.  In general, I think it is better to use an anonymized URL, or provide sample outputs as supplementary materials for double-blind reviewing.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 3
           Soundness / Correctness (1-5): 3
             Meaningful Comparison (1-5): 4
                      Thoroughness (1-5): 4
        Impact of Ideas or Results (1-5): 4
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
The authors propose a software toolkit for several SDP tasks. It is made
freely available online. As a modular architecture is chosen and
existing, well established components are being used, the general
approach taken seems sound. Referring to recent related work, the
authors properly position their work within the context of existing
literature. The key points of motivation for developing a new software
are (1) existing software being either too general (no SDP focus) or too
specific (e.g. for a certain scientific domain), and (2) the fact that
existing software is argued to be insufficiently accessible.
Pre-trained models integrated in the toolkit are evaluated against
existing approaches, where the proposed software is observed to achieve
a performance close to the state of the art. Given that SOTA components
appear to be integrated as is, this isn't much of a surprise.

In terms of presentation the proposed toolkit is described clearly and
the document structure is sound. Parts of section 2, however, read a bit
like a software documentation. Maybe the section could have been more
concise and the freed up space then used to discuss other aspects like
the toolkit's extensibility (e.g. ease of adding in a new data set or
embedding model).

While part of the motivation is the domain specificity of existing
software, some components of the proposed toolkit (for ScienceIE, I2B2,
and NER) appear to be domain specific as well.

Lastly, section 4 ends somewhat abruptly. A little discussion concerning
the listed use cases would have been helpful.

Overall, the presented work seems solid, but it is somewhat hard to give
a clear verdict, as no useful quantitative comparison to existing
software seems possible. The paper might be worth accepting, because the
tool appears useful and it would be interesting to see the community's
take on it.

Minor points:
- In Table 2 the toolkit is called "SciWING" instead of "SYS"
- Typo at the end of section 5: "provide access" -> "provides access"
---------------------------------------------------------------------------


Questions for Authors
---------------------------------------------------------------------------
1. Concerning datasets you argue that your toolkit unifies various input
formats. Can you elaborate on what this means for integrating further
data sets into the toolkit?
2. What was the reason for choosing the TOML format for configuration files?
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #3
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 5
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 4
           Soundness / Correctness (1-5): 5
             Meaningful Comparison (1-5): 5
                      Thoroughness (1-5): 4
        Impact of Ideas or Results (1-5): 4
                    Recommendation (1-5): 4
               Reviewer Confidence (1-5): 4

Detailed Comments
---------------------------------------------------------------------------
I would have appreciated a more in-depth analysis of the scalability/efficiency of SYS (currently and in the future), when facing processing of very large amounts of documents.
---------------------------------------------------------------------------

==> comments/comments.tex <==
Reviewer question ends in ---------
Our response ends in ========

---START---

Lastly, section 4 ends somewhat abruptly. A little discussion concerning
the listed use cases would have been helpful.
-----------------------------------------------------------------------------------------
 Abhi - Added one paragraph at the end of section 4 to conclude 
=====================================================================================


I was also not clear on what SciWING offers that differs from the base capabilities in AllenNLP.  Most of what the paper mentions in Section 2 -- the models, the training and testing capability, tokenizers, logging, metrics, support for embeddings, seem like AllenNLP components.  The TOML configuration file seems like an analogue to AllenNLP configuration files, albeit in a slightly different format.  Taking capabilities from AllenNLP makes perfect sense -- but the paper needs to be much more clear on what capabilities are new in this tool, versus built-in to AllenNLP.
---------------------------------------------------------------------------------------
Abhi - Addressed this by saying that we want to encourage researchers to minimally change an architecture and experiment vs AllenNLP which expects researcher to understand complex abstractions
=========================================================================================



What was the reason for choosing the TOML format for configuration files?
-------------------------------------------------------------------------------------
Abhi - It is widely used and is easy to read
========================================================================================


The tool aims to provide immediate access to SOTA models for scientific NLP.  My main concern with the paper is that the main claimed benefit with respect to other toolkits is that it provides access to SOTA models (with respect to those provided by other toolkits like AllenNLP, SciSpaCy, etc.)  But the paper doesn't include any empirical results to support this claim.  Also, I assume these are all moving targets as different toolkits incorporate new and better models.
----------------------------------------------------------------------------------------
Abhi: I agree in many cases they are not comparable. But in Citation intent classification we are 0.5 behind the state of the art without attention. I2B2 as well.
Addressed some of them in section 3.
==============================================================================================

---END----



==> sections/development_roadmap.tex <==
% Min: distributing this into your conclusion to save space.
% Currently this text is unused.
\section{Development Road Map}

\sciwing{} is developed actively. The project continues to add more models related to scientific document processing. We continue to support a wide range of transformers and other embeddings suitable for scientific document processing. Currently, \sciwing{} does not include models for sequence to sequence generation and we will be including it in the future releases of \sciwing{}. We also plan to include multi-task learning that has proven to be useful in scientific document processing that faces the challenge of small amounts of training data. 

==> sections/tasks.tex <==
% \section{Example Tasks}
% \sciwing{} includes examples for various task  which finds wide-spread use in scientific document processing. The examples demonstrate how to use the framework effectively. The models have verified performance levels that closely match the performance of the original results. They can be used as baselines for further research.

\begin{itemize}
    \item \textbf{Logical Structure Recovery} - Identifying the different logical sections of a research article like the introduction, conclusion, methodology experiments and others can aid in many downstream task like summarization, citation intent classification amongst others. Currently there are no neural network methods for logical structure recovery. We use the same dataset as \cite{kan}
    Examples neural network models which can serve as baselines for future research are included in \sciwing{}. 
    \textbf{\item Citation String Parsing} - Citation string parsing identifies the different parts of a citation string like the author of the research article, the journal and the year of publication and other data. Neural network methods for citation string parsing has shown good promise \cite{prasadanimesh}.  Citation string parsing is a sequence labelling task and \cite{prasadanimesh} combines a bidirectional LSTM with CRF. \sciwing{} includes the same architecture but also combines with ELMo embeddings.
    \textbf{\item ScienceIE task} - The task is to identify the different key-phrases in a scientific document. There are three key-phrases to be identified. Task key-phrases that denote the end task or goal, the material key-phrases indicate any chemical, dataset that is being used by the scientific work and the process includes any scientific model or algorithm. The state of the art system from 2017 includes a bidirectional LSTM with CRF and uses language model embeddings. \sciwing{} includes a reference implementation for the model but uses ELMo embeddings instead of the language model representations.
\end{itemize}

Other models are being actively developed for scientific document processing. We expect, that the development of these models is swift and easy and steadily grows over time.  The example implementations of these models can be found at \url{https://github.com/abhinavkashyap/sciwing/examples}.
